HeySQuAD: A Spoken Question Answering Dataset

Spoken question answering (SQA) systems are critical for digital assistants and other real-world use cases, but evaluating their performance is a challenge due to the importance of human-spoken questions. This study presents a new large-scale community-shared SQA dataset called HeySQuAD, which includes 76k human-spoken questions, 97k machine-generated questions, and their corresponding textual answers from the SQuAD QA dataset. Our goal is to measure the ability of machines to accurately understand noisy spoken questions and provide reliable answers. Through extensive testing, we demonstrate that training with transcribed human-spoken and original SQuAD questions leads to a significant improvement (12.51%) in answering human-spoken questions compared to training with only the original SQuAD textual questions. Moreover, evaluating with a higher-quality transcription can lead to a further improvement of 2.03%. This research has significant implications for the development of SQA systems and their ability to meet the needs of users in real-world scenarios.

==> sections/LLM.tex <==
In this section, we measure the ability of Large Language Models (LLM) including ChatGPT, GPT-4 to correct errors in the transcribed human-spoken questions and correspondingly the roberta-large QA model results.


==> sections/discussions.tex <==
\iffalse
can line 497 onwards be grouped under discussion? Yes! lets do that 
Will move this to error analysis! Done! (error_analysis.tex)
 is this last part refering to spoken squad?
 Yes
 Should we say that?
 It is an interesting challenge but maybe not? Its like giving shout out to Spoken Squad. 
  We performed some exploratory analysis to this effect using BERT-style models but noticed a significant decrease in performance. isnt this the one?
  hmm I see ok. 
 %In the previous sections, we benchmarked \digi\ dataset with several models and approches. But there are several more that could be employed to improve the accuracy given that \digi\, also has audio files accompanying the textual questions. This opens the door to experiment with audio-textual multi-modal models to get better at handling transcription errors by improving the ASR. The other approach could be to use both speech and text to directly query the answer from the textual context. That other avenue opens up when we join Spoken \squad\ and \digi. This simulates another real world scenario where the context and questions are transcribed from speech. When our models (roberta and albert based models) were trained on this joined dataset, we saw a significant decrease in performance.  
 \fi

==> sections/error_analysis.tex <==


% Say that the micro analysis is in agreement with macro analysis
\begin{table}
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}

\cline{1-3} ASR Transcription Error & WER & BLEU  \\ 
\cline{1-3}
 \digih \ Train by librispeech  & 0.3422 & 0.5303  \\ 
 \digih \ Dev librispeech & 0.2722  &  0.5914\\ 
  \digih \ Train by whisper  & 0.1088 & 0.8317  \\ 
 \digih \ Dev by whisper & 0.0471  & 0.8475 \\ 
\cline{1-3}
\end{tabular}%
}
\caption{WER and BLEU of transcribed human-spoken questions by librispeech and whisper ASR models.}\label{table:WER_BLEU_whisper}
\end{table}

\begin{table*}[t]
\centering
\resizebox{15cm}{!}{%
\begin{tabular}{{|c|c|c|c|c|c|}}
\hline
\textbf{QA Model}&& \textbf{Train Dataset}& \textbf{Val Dataset} & \textbf{F1}&\textbf{EM}\\ 
\hline
\multirow{10}{*}{\makecell{roberta-large}} &a& \squad\    train      and   \digih \ train by librispeech &          \digih \ dev by librispeech                 & 90.18 &	83.73 	\\ 
                                 &b    &\squad\    train      and   \digih \ train by librispeech &          \digih \ dev by whisper                 & 92.19&	85.33 	\\ 
                                &c   & \squad\    train      and   \digih \ train by whisper &          \digih \ dev by librispeech                 &  84.75&76.35	\\ 
                                 &d  &  \squad\    train      and   \digih \ train by whisper &          \digih \ dev by whisper              &  91.21 & 83.23 	\\ 
                                 &e  &  \squad\    train    &          \digih \ dev by librispeech                 & 77.67	& 63.87	\\ 
                                 &f  &  \squad\    train   &          \digih \ dev by whisper                 & 92.15	& 84.63 	\\ 
                                 &g  &  \digih \ train by librispeech    &          \digih \ dev by librispeech                 &  89.14& 81.93	  	\\ 
                                 &h  &  \digih \ train by librispeech   &          \digih \ dev by whisper                 & 92.21 	&  84.43 	\\ 
                                 &i  &  \digih \ train by whisper    &          \digih \ dev by librispeech                 & 84.70 	&  76.85	\\ 
                                 &j  &  \digih \ train by whisper   &          \digih \ dev by whisper                 & 90.49 	&  82.83 	\\ 
                                  \hline
\end{tabular}%
}
\caption{QA accuracy results (\%) using roberta-large QA models fine-tuned on \digih and \squad\ train dataset using two different ASR models: librispeech and whisper.}\label{table:QA_results_whisper}
\end{table*}


% Continue with different types of transcription errors  (who/what analysis) [waiting for some data]



% Discussions
 %The primary goal of \digi\ is to develop a dataset for SQA that allows us to build models that help understand noisy spoken questions and answer them accurately. 

%should we say discussions in bold as a title on 497? Or here. 

% is that good? (line 147 of this doc)






























==> sections/evaluation.tex <==
\subsection{Evaluation Metrics}

With the ASR transcriptions of human-spoken and machine-generated questions,
the Question Answering models can return a text answer
based on the questions and contexts. Since the task involves retrieval of a span of text, we employ two types of evaluation metrics to gauge the performance of models: (1) Computing the exact match(EM) between the predicted text answer and the ground truth text answer and (2) F1 scores between the predicted text answer and the ground-truth text answer. For instance, if the predicted text answer is exactly the same as the ground-truth text answer the EM score is 1 and F1 is 1. However, when there is a mismatch between them, EM score is 0 where are F1 scores are between 0 and 1. The F1 score is based on the precision and recall. Precision is the percentage of words in the predicted answer existing in the ground-truth answer, while the recall is the percentage of words in the ground-truth answer also appearing in the predicted answer.

==> sections/limitations.tex <==
\textbf{Limitations.} We use only the transcription of the audio files in our models, and we do not build models directly with audio files in the dataset. The SQA models we build contain ASR errors which percolate thru other modules, leading to error propagation.  \\
\textbf{Potential Risks.} A fully realized SQA system might pose privacy risks to the end customer.  \\
\textbf{Impact.} We present HeySQuAD that includes both human-spoken and machine-generated audio and transcribed questions. This will help future researchers study various effects of variability in human speech and design approaches to alleviate spurious trasncriptions. 

==> sections/old_machine_digi_exp_results.tex <==
\begin{table*}
 \caption{BERT,RoBERTa,ALBERT QA model fine-tuned on \squad\ 1.1}
  \centering
  \begin{adjustbox}{width=1\textwidth}
  \small
  \begin{tabular}{|c|c|c|c|c|c|}
    \toprule
    \multirow{2}{*}{Model} &\multirow{2}{*}{fine-tuned dataset} & \multicolumn{2}{c}{\squad\ 1.1 Dev} &\multicolumn{2}{c}{\digi\  1.1 Dev}\\
                        &                                          & F1  & EM & F1 & EM\\
    \toprule
    \multirow{4}{*}{bert-base-uncased(QuASR)} & \squad\ 1.1 train &	88.2&	80.9&	67.7&	52.4   \\
                                            &   \digi\ 1.1 train &	 &	 &	84.4&	76.6   \\
                                             &  \squad\ 1.1 train and \digi\ 1.1 train &	 &	 &	84.5&	76.1   \\
                                            &   \squad\ 1.1 train and then \digi\ 1.1 train &	 &	&	84.3&	76.2   \\
                                            &  with MSE alignment loss &	 &	 &	85.6&78.2	   \\
                                            &  with CosSim alignment loss &	 &	 &85.5	&78.0	   \\
    \midrule
    \multirow{4}{*}{bert-large-uncased(QuASR)} & \squad\ 1.1 train &	93.4&	83.1&	74.0&	64.7   \\
                                            &   \digi\ 1.1 train &	 &	& 87.0&	79.6   \\
                                             &  \squad\ 1.1 train and \digi\ 1.1 train &	&	&	86.8&	79.0  \\
                                            &   \squad\ 1.1 train and then \digi\ 1.1 train &	&	&87.0	&79.2   \\
                                            &  with MSE alignment loss &	 &	 &	88.0&81.0	   \\
                                            &  with CosSim alignment loss &	 &	 &87.6	&80.6	   \\
    \midrule
    \multirow{4}{*}{albert-base-v2(QuASR)} & \squad\ 1.1 train &	89.9&	82.4&	71.6&	55.4   \\
                                            &   \digi\ 1.1 train &	 &	&	87.2& 79.7   \\
                                             &  \squad\ 1.1 train and \digi\ 1.1 train &	& &	 85.3&	77.5  \\
                                            &   \squad\ 1.1 train and then \digi\ 1.1 train &	& &	86.3&	78.5   \\
                                            &  with MSE alignment loss &	 &	 &86.1	& 78.6	   \\
                                            &  with CosSim alignment loss &	 &	 &85.0 &77.5 	   \\
    \midrule
    \multirow{4}{*}{albert-large-v2(QuASR)} & \squad\ 1.1 train &	92.3&	85.7&	67.5&	47.9   \\
                                            &   \digi\ 1.1 train &	& &	89.6&	82.6  \\
                                             &  \squad\ 1.1 train and \digi\ 1.1 train &	& & 	89.6&	82.7   \\
                                            &   \squad\ 1.1 train and then \digi\ 1.1 train & & & 88.2& 80.8  \\
                                            &  with MSE alignment loss &	 &	 &	88.2& 80.9	   \\
                                            &  with CosSim alignment loss &	 &	 &88.0	& 80.8   \\
    \midrule
    \multirow{4}{*}{roberta-base(QuASR)} & \squad\ 1.1 train &91.1 & 84.3&83.3 &75.0   \\
                                            &   \digi\ 1.1 train &	& & 88.3&81.5    \\
                                             &  \squad\ 1.1 train and \digi\ 1.1 train & & &87.0 & 79.3 \\
                                            &   \squad\ 1.1 train and then \digi\ 1.1 train & & & 87.9&80.3   \\
                                             &  with MSE alignment loss &	 &	 &	88.7&81.8	   \\
                                            &  with CosSim alignment loss &	 &	 &88.4&81.4	   \\
    \midrule
    \multirow{4}{*}{roberta-large(QuASR)} & \squad\ 1.1 train &	92.3&	85.6&	82.3&	71.2    \\
                                            &   \digi\ 1.1 train & & &	91.9&	85.5   \\
                                             &  \squad\ 1.1 train and \digi\ 1.1 train & & &	91.7&	84.9  \\
                                            &   \squad\ 1.1 train and then \digi\ 1.1 train & & &	90.7&	84.0   \\
                                            &  with MSE alignment loss &	 &	 &90.8	& 84.4   \\
                                            &  with CosSim alignment loss &	 &	 &91.0 & 	84.5   \\
                                            



    \toprule
    JoiQA & -& - & - & 26.77 & 35.65 \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{table_results}
\end{table*}

%NMT result
\begin{table*}
 \caption{BERT,RoBERTa,ALBERT QA model applied on NMT-\digi\ 1.1 Dev}
  \centering
  \begin{tabular}{|c|c|c|c|}
    \toprule
    \multirow{2}{*}{Model} &\multirow{2}{*}{fine-tuned dataset} &\multicolumn{2}{c}{NMT-\digi\ 1.1 Dev}\\
                        & & F1 & EM\\
    \toprule
    \multirow{2}{*}{bert-base-uncased(QuASR)} & \squad\ 1.1 train &84.1&	76.3 \\
                                            &   \digi\ 1.1 train &	 84.5	&76.4   \\
    \midrule
    \multirow{2}{*}{bert-large-uncased(QuASR)} & \squad\ 1.1 train &	87.9&	80.6   \\
                                            &   \digi\ 1.1 train & 87.1&	79.7   \\
    \midrule
    \multirow{2}{*}{albert-base-v2(QuASR)} & \squad\ 1.1 train &85.2	& 77.4  \\
                                            &   \digi\ 1.1 train &	87.0&79.6   \\
    \midrule
    \multirow{2}{*}{albert-large-v2(QuASR)} & \squad\ 1.1 train &	87.9&	80.6\\
                                            &   \digi\ 1.1 train &89.3	& 82.3  \\
    \midrule
    \multirow{2}{*}{roberta-base(QuASR)} & \squad\ 1.1 train & 86.9 &  79.9 \\
                                            &   \digi\ 1.1 train &88.1	&81.0     \\
    \midrule
    \multirow{2}{*}{roberta-large(QuASR)} & \squad\ 1.1 train &	88.6&	81.7    \\
                                            &   \digi\ 1.1 train &89.9 &83.1    \\
                                            



    \bottomrule
  \end{tabular}
  \label{table_results}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}
\caption{Digi ASR Model 1 (facebook/s2t-small-librispeech-asr) WER}

\begin{tabular}{|c|c|}
\toprule
\textbf{ASR Transcription Error}     &  \textbf{WER(0-1)}  \\ 
\midrule

\squad\ 1.1 Dev set questions VS \digi\ 1.1 Dev set transcribed questions           & 0.31                                                               \\ 
\midrule
\squad\ 1.1 Training set questions VS \digi\ 1.1 Training set transcribed questions & 0.21                                                               \\ 
\bottomrule

\end{tabular}
\end{table*}




\begin{table*}
\caption{BERT,RoBERTa,ALBERT QA model fine-tuned on transcribed contexts and transcribed questions}
\begin{tabular}{|c|c|cc|cc|}
\hline
\multirow{2}{*}{Model}              & \multirow{2}{*}{Fine-tuned Dataset} & \multicolumn{2}{c|}{\squad\ 1.1 Dev} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Transcribed Context and\\  Question \squad\ 1.1 Dev\end{tabular}} \\
                                    &                                              & \multicolumn{1}{c|}{F1}        & EM        & \multicolumn{1}{c|}{F1}                                              & EM                                              \\ \hline
\multirow{2}{*}{bert-base-uncased}  & \squad\ 1.1                                     & \multicolumn{1}{c|}{88.4}      & 81.0      & \multicolumn{1}{c|}{46.1}                                            & 27.1                                            \\
                                    & Transcribed Context and Question \squad\ 1.1    & \multicolumn{1}{c|}{72.7}      & 59.6      & \multicolumn{1}{c|}{52.8}                                            & 38.3                                            \\ \hline
\multirow{2}{*}{bert-large-uncased} & fine-tuned on \squad\ 1.1                       & \multicolumn{1}{c|}{90.4}     & 83.1     & \multicolumn{1}{c|}{48.1}                                           & 28.3                                           \\
                                    & Transcribed Context and Question \squad\ 1.1    & \multicolumn{1}{c|}{78.7}     & 65.6     & \multicolumn{1}{c|}{54.9}                                           & 40.3                                           \\ \hline
\multirow{2}{*}{roberta-base}       & \squad\ 1.1                                     & \multicolumn{1}{c|}{91.4}      & 84.5      & \multicolumn{1}{c|}{49.8}                                            & 30.1                                            \\
                                    & Transcribed Context and Question \squad\ 1.1    & \multicolumn{1}{c|}{71.4}      & 30.6      & \multicolumn{1}{c|}{50.1}                                            & 13.5                                            \\ \hline
\multirow{2}{*}{roberta-large}      & fine-tuned on \squad\ 1.1                       & \multicolumn{1}{c|}{92.3}      & 85.6      & \multicolumn{1}{c|}{51.5}                                            & 30.6                                            \\
                                    & Transcribed Context and Question \squad\ 1.1    & \multicolumn{1}{c|}{75.2}      & 31.0      & \multicolumn{1}{c|}{53.4}                                            & 14.6                                            \\ \hline
\multirow{2}{*}{albert-base-v2}     & \squad\ 1.1                                     & \multicolumn{1}{c|}{90.4}      & 83.3      & \multicolumn{1}{c|}{46.2}                                            & 25.8                                            \\
                                    & Transcribed Context and Question \squad\ 1.1    & \multicolumn{1}{c|}{78.0}      & 64.6      & \multicolumn{1}{c|}{57.5}                                            & 43.4                                            \\ \hline
\multirow{2}{*}{albert-large-v2}    & fine-tuned on \squad\ 1.1                       & \multicolumn{1}{c|}{92.4}      & 85.7      & \multicolumn{1}{c|}{43.1}                                            & 20.8                                            \\
                                    & Transcribed Context and Question \squad\ 1.1    & \multicolumn{1}{c|}{80.6}      & 66.5      & \multicolumn{1}{c|}{57.0}                                            & 42.5                                            \\ \hline
\end{tabular}
\end{table*}


\begin{table*}
\caption{Context ASR Model 2 (facebook/wav2vec2-conformer-rope-large-960h-ft) WER}
\begin{tabular}{|c|c|c}
\toprule
\textbf{ASR Transcription Error}                                                    & \textbf{WER(0-1)}  \\
\midrule

\squad\ 1.1 Dev set questions VS \digi\ 1.1 Dev set transcribed questions           & 0.1618              \\
\midrule

\squad\ 1.1 Training set questions VS \digi\ 1.1 Training set transcribed questions & 0.1554            \\
\midrule
\squad\ 1.1 Dev set contexts VS \digi\ 1.1 Dev set transcribed contexts           & 0.2132             \\
\midrule
\squad\ 1.1 Training set contexts VS \digi\ 1.1 Training set transcribed contexts & 0.2165            \\
\bottomrule

\end{tabular}
\end{table*}



==> sections/task_description.tex <==
% TODO: take another pass
We are interested in the task of spoken query answering (SQA). Specifically, given a spoken query and a passage that contains answer to the query, the objective is to identify the answer to the query. In this paper, we present an initial attempt towards formalizing this problem. As first phase,  we take a machine comprehension dataset like \squad\ and reframe the dataset to make it suitable for voice based query answering. We create a dataset called \digi\ and then propose models architectures to solve the task of Spoken Question Answering.

